Outflows and the Physical Properties of Quasars

We have investigated a sample of 5088 quasars from the Sloan Digital Sky Survey Second Data Release in order to determine how the frequency and properties of broad absorptions lines (BALs) depend on black hole mass, bolometric luminosity, Eddington fraction (L/L_Edd), and spectral slope. We focus only on high-ionization BALs and find a number of significant results. While quasars accreting near the Eddington limit are more likely to show BALs than lower $L/L_{Edd}$ systems, BALs are present in quasars accreting at only a few percent Eddington. We find a stronger effect with bolometric luminosity, such that the most luminous quasars are more likely to show BALs. There is an additional effect, previously known, that BAL quasars are redder on average than unabsorbed quasars. The strongest effects involving the quasar physical properties and BAL properties are related to terminal outflow velocity. Maximum observed outflow velocities increase with both the bolometric luminosity and the blueness of the spectral slope, suggesting that the ultraviolet luminosity to a great extent determines the acceleration. These results support the idea of outflow acceleration via ultraviolet line scattering.

==> tab4.tex <==
\begin{deluxetable}{lcccccccccccc}
%\rotate
\tablewidth{0pc}
\tabletypesize{\tiny}
%
\tablecaption{Measured and Derived Quasar Parameters}
%
\tablehead {
\colhead{Name} &
\colhead{MJD} &
\colhead{Plate} &
\colhead{Fiber} &
\colhead{Redshift} &
\colhead{$F_\lambda$} &
\colhead{$\alpha_\mathrm{NUV}$} &
\colhead{$\lambda L_\lambda$} &
\colhead{\ion{Mg}{2}} &
\colhead{$M_\mathrm{BH}$} &
\colhead{$L_\mathrm{bol}/$} &
\colhead{Run} &
\colhead{Class} \\
 & & & & & & & &
\colhead{FWHM} & & \colhead{$L_\mathrm{Edd}$}
}
\startdata
SDSS J000009.42-102751.88 & 52143 & 0650 & 199 & 1.844230  & 2.2672 & 1.802 &  4.577 & 12320 &  30.86 & 0.0578 & 2 & AAL \\
SDSS J000058.24-004646.29 & 51791 & 0387 & 093 & 1.895120  & 2.9567 & 1.763 &  6.496 &  4560 &  4.983 & 0.5182 & 1 & Reg \\
SDSS J000118.42-010221.60 & 51791 & 0387 & 042 & 1.968500  & 1.2266 & 1.843 &  3.033 &  9200 &  14.18 & 0.0815 & 3 & AAL \\
SDSS J000119.64+154828.78 & 52235 & 0750 & 566 & 1.924210  & 2.3214 & 1.301 &  5.347 &  4885 &  5.219 & 0.5205 & 3 & BAL \\
SDSS J000139.43+152624.11 & 52235 & 0750 & 541 & 1.789660  & 5.8318 & 1.246 &  10.73 &  4370 &  5.793 & 0.9685 & 1 & Reg \\
SDSS J000139.64-103824.05 & 52143 & 0650 & 136 & 1.820630  & 1.9547 & 1.017 &  3.792 &  4300 &  3.441 & 0.6511 & 2 & Reg \\
SDSS J000219.34-105259.58 & 52143 & 0650 & 097 & 1.762000  & 0.9093 & 0.436 &  1.594 &  5245 &  3.406 & 0.3763 & 2 & AAL \\
SDSS J000221.80+151454.59 & 52235 & 0750 & 553 & 1.823530  & 3.3027 & 1.123 &  6.438 &  3840 &  3.519 & 1.0215 & 3 & AAL \\
SDSS J000319.87-090156.19 & 52143 & 0650 & 561 & 1.760220  & 9.9334 & 1.637 &  17.36 &  3390 &  4.371 & 1.6877 & 3 & Reg \\
SDSS J000422.30-090219.36 & 52143 & 0650 & 609 & 1.858810  & 5.1395 & 1.323 &  10.63 &  3370 &  3.431 & 1.5558 & 2 & Reg \\
SDSS J000510.84-092534.79 & 52143 & 0650 & 621 & 1.866540  & 1.6132 & 1.170 &  3.381 &  3635 &  2.330 & 0.7906 & 3 & Reg \\
SDSS J000546.49-002413.98 & 51793 & 0388 & 268 & 1.729750  & 2.0840 & 1.133 &  3.450 &  3705 &  2.443 & 0.7843 & 3 & Reg \\
SDSS J000612.30-104310.65 & 52141 & 0651 & 258 & 1.735310  & 3.3973 & 1.481 &  5.680 &  3455 &  2.686 & 0.9767 & 2 & Reg \\
SDSS J000629.29-093550.93 & 52141 & 0651 & 429 & 1.758180  & 5.0479 & 0.936 &  8.788 &  6880 &  13.08 & 0.4144 & 2 & Reg \\
SDSS J000648.74-094037.00 & 52141 & 0651 & 468 & 1.835040  & 2.5152 & 0.686 &  5.000 &  3970 &  3.340 & 1.0543 & 2 & AAL \\
SDSS J000654.11-001533.30 & 51793 & 0388 & 234 & 1.725170  & 7.5664 & 0.943 &  12.42 &  4650 &  7.028 & 1.0857 & 4 & Reg \\
SDSS J000735.52-085435.16 & 52141 & 0651 & 417 & 1.777750  & 2.4386 & 1.561 &  4.394 &  3315 &  2.191 & 0.8873 & 2 & Reg \\
SDSS J000759.40+150822.65 & 52251 & 0751 & 557 & 1.968020  & 2.4355 & 0.887 &  6.017 &  2915 &  1.964 & 1.9385 & 2 & Reg \\
SDSS J000815.33-095854.03 & 52141 & 0651 & 494 & 1.949790  & 6.6211 & 0.854 &  15.89 &  4420 &  7.129 & 1.4353 & 1 & AAL \\
SDSS J000904.43-004332.85 & 51793 & 0388 & 098 & 1.828630  & 3.8336 & 1.089 &  7.538 &  3700 &  3.518 & 1.2179 & 4 & Reg \\
SDSS J000919.26+152355.17 & 52251 & 0752 & 343 & 1.934950  & 1.4671 & 1.883 &  3.439 &  4730 &  3.976 & 0.3226 & 2 & AAL \\
SDSS J001017.52-100238.90 & 52138 & 0652 & 316 & 1.819020  & 2.8847 & 1.216 &  5.581 &  4075 &  3.705 & 0.8005 & 2 & AAL \\
SDSS J001017.81+010450.74 & 51793 & 0388 & 607 & 1.817960  & 3.6331 & 0.992 &  7.016 &  5120 &  6.514 & 0.6446 & 3 & AAL \\
SDSS J001020.25-103059.09 & 52141 & 0651 & 107 & 1.742540  & 2.5056 & 1.424 &  4.243 &  5045 &  4.993 & 0.4045 & 3 & AAL \\
SDSS J001029.92-101145.54 & 52138 & 0652 & 302 & 1.751640  & 3.2360 & 1.281 &  5.569 &  3665 &  2.994 & 0.9550 & 1 & Reg \\
SDSS J001053.58+000642.84 & 51795 & 0389 & 348 & 1.873370  & 2.6721 & 1.169 &  5.664 &  5655 &  7.185 & 0.4296 & 3 & Reg \\
SDSS J001054.41-085438.66 & 52141 & 0651 & 569 & 1.745720  & 9.3966 & 1.043 &  16.00 &  4485 &  7.364 & 1.2662 & 4 & Reg \\
SDSS J001111.14+151034.83 & 52251 & 0751 & 632 & 1.731630  & 2.7532 & 1.609 &  4.573 &  5700 &  6.602 & 0.2989 & 1 & Reg \\
SDSS J001142.79+152216.30 & 52251 & 0752 & 438 & 1.886190  & 3.6573 & 0.219 &  7.918 &  3270 &  2.812 & 2.5391 & 4 & Reg \\
SDSS J001157.76-103735.21 & 52138 & 0652 & 264 & 1.857680  & 4.2954 & 0.774 &  8.870 &  4060 &  4.573 & 1.3031 & 4 & AAL \\
SDSS J001244.62+141112.97 & 52251 & 0752 & 217 & 1.705560  & 3.2471 & 0.842 &  5.146 &  5660 &  6.881 & 0.4847 & 4 & AAL \\
SDSS J001330.58+001814.28 & 51795 & 0389 & 385 & 1.844230  & 1.8880 & 1.713 &  3.812 &  4270 &  3.401 & 0.4575 & 2 & Reg \\
SDSS J001341.74+143531.31 & 52251 & 0752 & 194 & 1.933230  & 1.8982 & 1.433 &  4.437 &  6480 &  8.412 & 0.2499 & 3 & AAL \\
SDSS J001400.45+004255.49 & 51795 & 0389 & 412 & 1.709720  & 4.5593 & 1.438 &  7.280 &  4045 &  4.137 & 0.8314 & 3 & Reg \\
SDSS J001408.23-085242.19 & 52138 & 0652 & 363 & 1.744560  & 4.5117 & 0.137 &  7.668 &  6825 &  12.07 & 0.5987 & 2 & BAL \\
SDSS J001411.00-084429.15 & 52138 & 0652 & 375 & 1.767220  & 2.9899 & 0.287 &  5.289 &  5470 &  6.510 & 0.7068 & 2 & AAL \\
SDSS J001438.28-010750.12 & 51795 & 0389 & 211 & 1.815640  & 4.8011 & 0.553 &  9.234 &  3295 &  3.070 & 2.2729 & 2 & BAL \\
SDSS J001453.37-002827.52 & 51795 & 0389 & 239 & 1.922620  & 3.7010 & 0.566 &  8.503 &  4405 &  5.278 & 1.2093 & 2 & Reg \\
SDSS J001507.00-000800.81 & 51795 & 0389 & 196 & 1.703300  & 10.118 & 0.906 &  15.97 &  3020 &  3.336 & 2.9997 & 1 & Reg \\
SDSS J001545.33-095754.12 & 52138 & 0652 & 479 & 1.795910  & 1.3341 & 1.949 &  2.481 &  4780 &  3.483 & 0.2565 & 2 & Reg \\
SDSS J001657.00+005532.06 & 51900 & 0390 & 331 & 1.756100  & 3.0960 & 1.595 &  5.370 &  3775 &  3.123 & 0.7474 & 3 & Reg \\
SDSS J001710.85+135556.52 & 52251 & 0752 & 044 & 1.808170  & 10.460 & 1.386 &  19.86 &  4360 &  7.704 & 1.2523 & 1 & AAL \\
SDSS J001741.85-105613.30 & 52138 & 0652 & 041 & 1.806080  & 3.6452 & 1.407 &  6.897 &  3555 &  3.115 & 1.0631 & 2 & Reg \\
SDSS J001800.21+004602.82 & 51795 & 0389 & 611 & 1.900380  & 3.3131 & 1.584 &  7.342 &  4690 &  5.583 & 0.5749 & 2 & Reg \\
SDSS J001826.80-091038.78 & 52138 & 0652 & 578 & 1.857870  & 2.9839 & 0.911 &  6.164 &  4105 &  3.940 & 0.9775 & 2 & Reg \\
SDSS J001913.57-103848.25 & 52138 & 0652 & 070 & 1.862490  & 2.2511 & 0.822 &  4.686 &  4245 &  3.704 & 0.8289 & 4 & Reg \\
SDSS J001959.48-090809.46 & 52145 & 0653 & 324 & 1.792750  & 1.4842 & 1.450 &  2.745 &  6195 &  6.135 & 0.2100 & 3 & Reg \\
SDSS J002000.50+155110.02 & 52233 & 0753 & 374 & 1.751000  & 1.9210 & 1.737 &  3.302 &  4470 &  3.484 & 0.3821 & 3 & AAL \\
SDSS J002028.35-002915.00 & 51900 & 0390 & 234 & 1.926880  & 2.7439 & 1.765 &  6.348 &  4165 &  4.112 & 0.6132 & 2 & AAL \\
SDSS J002028.97+153435.91 & 52233 & 0753 & 430 & 1.764390  & 4.2464 & 1.156 &  7.474 &  4035 &  4.168 & 0.9841 & 2 & AAL \\
SDSS J002127.88+010420.39 & 51900 & 0390 & 443 & 1.819400  & 4.9046 & 1.518 &  9.494 &  7615 &  16.61 & 0.2588 & 2 & BAL \\
SDSS J002132.63-092424.31 & 52145 & 0653 & 422 & 1.869800  & 2.8025 & 1.081 &  5.905 &  5690 &  7.419 & 0.4545 & 3 & Reg \\
SDSS J002143.30+010840.26 & 51900 & 0390 & 534 & 1.901220  & 2.2417 & 1.618 &  4.974 &  4790 &  4.850 & 0.4404 & 3 & Reg \\
SDSS J002302.56+153446.39 & 52233 & 0753 & 462 & 1.723460  & 3.2186 & 1.294 &  5.268 &  4790 &  4.983 & 0.5393 & 2 & BAL \\
SDSS J002344.36+143115.43 & 52233 & 0753 & 165 & 1.866000  & 5.4223 & 1.334 &  11.35 &  7715 &  18.54 & 0.3056 & 1 & BAL \\
SDSS J002411.66-004348.06 & 51782 & 0391 & 290 & 1.794470  & 6.6288 & 1.839 &  12.29 &  4575 &  6.770 & 0.6936 & 3 & AAL \\
SDSS J002439.64-091600.58 & 52145 & 0653 & 538 & 1.792960  & 3.5242 & 1.638 &  6.519 &  4625 &  5.135 & 0.5395 & 3 & Reg \\
SDSS J002448.07-090055.05 & 52145 & 0653 & 530 & 1.858650  & 3.2093 & 1.476 &  6.638 &  4510 &  4.924 & 0.6242 & 3 & Reg \\
\enddata
\tablecomments{{\it The full table is to appear in the electronic version only.} Units
on $F_\lambda$\ are $10^{-17}$\,erg cm$^{-2}$\ s$^{-1}$\ \AA$^{-1}$. Units on $\lambda
L_\lambda$\ are $10^{45}$\,erg s$^{-1}$. Both $F_\lambda$\ and $\lambda L_\lambda$\
are taken at 3000\,\AA. Units on the \ion{Mg}{2} FWHM are \kms. Units on $M_\mathrm{BH}$\ are
$10^8\,M_\odot$.}
\label{tab:qsos}
\end{deluxetable}

